Duoquest: A Dual-Specification System for Expressive SQL Queries

Querying a relational database is difficult because it requires users to know both the SQL language and be familiar with the schema. On the other hand, many users possess enough domain familiarity or expertise to describe their desired queries by alternative means. For such users, two major alternatives to writing SQL are natural language interfaces (NLIs) and programming-by-example (PBE). Both of these alternatives face certain pitfalls: natural language queries (NLQs) are often ambiguous, even for human interpreters, while current PBE approaches require either low-complexity queries, user schema knowledge, exact example tuples from the user, or a closed-world assumption to be tractable. Consequently, we propose dual-specification query synthesis, which consumes both a NLQ and an optional PBE-like table sketch query that enables users to express varied levels of domain-specific knowledge. We introduce the novel dual-specification Duoquest system, which leverages guided partial query enumeration to efficiently explore the space of possible queries. We present results from user studies in which Duoquest demonstrates a 62.5% absolute increase in query construction accuracy over a state-of-the-art NLI and comparable accuracy to a PBE system on a more limited workload supported by the PBE system. In a simulation study on the prominent Spider benchmark, Duoquest demonstrates a >2x increase in top-1 accuracy over both NLI and PBE.

==> plots/ablation.tex <==
\begin{figure}[t]
  \begin{subfigure}[b]{0.5\columnwidth}
    \centering
    \input{plots/ablation_dev.tex}
    \vspace{-0.5cm}
    \caption{\makebox[0.4cm][l]{Spider Dev}}
    \label{fig:ablation-dev}
  \end{subfigure}%
  \begin{subfigure}[b]{0.44\columnwidth}
    \centering
    \input{plots/ablation_test.tex}
    \vspace{-0.5cm}
    \caption{Spider Test}
    \label{fig:ablation-test}
  \end{subfigure}%
\caption{Distributions comparing \system\ with select verification components disabled. A higher curve indicates superior performance.}
\label{fig:ablation}
\end{figure}

==> tables/approaches.tex <==
\begin{table}[t]
  \centering
  \begin{tabular}{lp{4.4cm}cc}
    \toprule
        \textbf{Approach} & \textbf{Description} & \textbf{NLQ} & \textbf{TSQ} \\
    \midrule
        \system & Implements GPQE & \cmark & \cmark \\
        Chain & Alternative dual-specification approach. Verifies completed candidates, not partial queries. & \cmark & \cmark \\
        NLI & SyntaxSQLNet \cite{yu2018syntaxsqlnet}, modified as described in Section~\ref{sec:enumeration}. & \cmark & \\
        PBE & Enumerator in \system\ replaced with breadth-first search. Approximates state-of-the-art PBE. & & \cmark \\
    \bottomrule
  \end{tabular}
  \caption{Approaches compared in our simulation study. \cmark\ indicates whether the NLQ or TSQ specifications were provided as input to the system.}
  \label{tab:approaches}
%   \vspace{-0.8cm}
\end{table}

==> tables/tasks.tex <==
\begin{table*}[t]
  \centering
  \small
  \begin{tabular}{ccp{4.2cm}P{10.7cm}}
    \toprule
      \textbf{Task} & \textbf{Level} & \textbf{English Description} & \textbf{SQL} \\
    \midrule
      A1 & M & List all publications in conference C and their year of publication. & \texttt{SELECT t2.title, t2.year FROM conference AS t1 JOIN publication AS t2 ON t1.cid = t2.cid WHERE t1.name = 'C'}\\
      B4 & H & List authors from organization R with more than 50 publications and the number of publications for each author. & \texttt{SELECT t1.name, COUNT(*) FROM author AS t1 JOIN writes AS t2 ON t1.aid = t2.aid JOIN organization AS t3 ON t1.oid = t3.oid JOIN publication AS t4 ON t2.pid = t4.pid WHERE t3.name = 'R' GROUP BY t1.name HAVING COUNT(*) > 50} \\
      C2 & M & List authors in domain D. & \texttt{SELECT t1.name FROM author AS t1 JOIN domain\textunderscore author AS t2 ON t1.aid = t2.aid JOIN domain AS t3 ON t2.did = t3.did WHERE t3.name = 'D'} \\
      D3 & H & List authors with more than 8 papers in conference C. & \texttt{SELECT t1.name FROM author AS t1 JOIN writes AS t2 ON t1.aid = t2.aid JOIN publication AS t3 ON t2.pid = t3.pid JOIN conference AS t4 ON t3.cid = t4.cid WHERE t4.name = 'C' GROUP BY t1.name HAVING COUNT(t3.pid) > 8} \\
    \bottomrule
  \end{tabular}
  \caption{A subset of tasks from the user studies. Foreign key names and literal values are abbreviated for space reasons. English descriptions were not provided to users during the study. Full list of tasks in Appendix~\ref{appendix:tasks}.}
  \label{tab:tasks}
  \vspace{-0.4cm}
\end{table*}

==> tables/user_acc.tex <==
\begin{table}[t]
  \centering
  \begin{tabular}{cccccccc}
    \toprule
        & \multicolumn{3}{c}{\textbf{NLI}} & \multicolumn{4}{c}{\bfseries{\system}} \\
        \cmidrule(lr){2-4} \cmidrule(lr){5-8}
        \textbf{Task} & \cmark & \xmark & TO & \cmark & \xmark & TO & \# Ex. \\
    \midrule
        A1 & 5/8 & 2/8 & 1/8 & \textbf{8/8} & 0/8 & 0/8 & 1\\
        A2 & 1/8 & 1/8 & 6/8 & \textbf{5/8} & 0/8 & 3/8 & 1.13\\
        A3 & 0/8 & 1/8 & 7/8 & \textbf{6/8} & 0/8 & 2/8 & 1.25\\
        A4 & 0/8 & 0/8 & 8/8 & \textbf{8/8} & 0/8 & 0/8 & 1.38\\
        B1 & 5/8 & 1/8 & 2/8 & \textbf{8/8} & 0/8 & 0/8 & 1.25\\
        B2 & 2/8 & 0/8 & 6/8 & \textbf{8/8} & 0/8 & 0/8 & 1.13\\
        B3 & 2/8 & 1/8 & 5/8 & \textbf{8/8} & 0/8 & 0/8 & 1.5\\
        B4 & 0/8 & 0/8 & 8/8 & \textbf{4/8} & 0/8 & 4/8 & 1.5\\
    \bottomrule
  \end{tabular}
  \caption{Accuracy for each task on the user study. \cmark\ are attempts for which the correct query was selected, \xmark\ are attempts with incorrect query selections, TO is the number of times the user gave up or the timeout was reached, and \# Ex. is the average number of examples used for \system\ attempts for each task.}
  \label{tab:user-acc}
\end{table}
